Improving Gradient Estimation in Evolutionary Strategies With Past Descent Directions

Evolutionary Strategies (ES) are known to be an effective black-box optimization technique for deep neural networks when the true gradients cannot be computed, such as in Reinforcement Learning. We continue a recent line of research that uses surrogate gradients to improve the gradient estimation of ES. We propose a novel method to optimally incorporate surrogate gradient information. Our approach, unlike previous work, needs no information about the quality of the surrogate gradients and is always guaranteed to find a descent direction that is better than the surrogate gradient. This allows to iteratively use the previous gradient estimate as surrogate gradient for the current search point. We theoretically prove that this yields fast convergence to the true gradient for linear functions and show under simplifying assumptions that it significantly improves gradient estimates for general functions. Finally, we evaluate our approach empirically on MNIST and reinforcement learning tasks and show that it considerably improves the gradient estimation of ES at no extra computational cost.

==> oldstuff.tex <==

\subsection{old version of section 3}
Given an $N$-dimensional function $f:\mathbb{R}^N\to \mathbb{R}$ which we want to minimize. Assuming we do not have easy access to the gradient of $f$, we need to estimate it. For that end, we can easily estimate the gradient of $f$ in a particular direction $\eps$ by: 
$$
\frac{f(x+\eps) - f(x-\eps)}{2}\approx \ls \tri f(x), \eps \rs 
$$
where we assume in the approximation that third and higher order terms in the Taylor expansion of $f$ around $x$ can be ignored, that is, $f(x+\eps) \approx f(x)+ \ls\tri f(x), \eps\rs + \ls \eps , H \eps \rs$.

In low dimensional spaces, it would be easy to estimate the gradient by using the above estimate in an orthogonal basis that spans the subspace. In a high dimensional space, this is too costly and we have to settle for sampling in a subset of the space. Given orthogonal directions $\eps_i$ for $i$ from $1$ to $k$, we get an estimate of the partial derivative of $f$ in the direction of $\eps_i$ for each $i$. Given these estimates, the goal is to combine the information in these partial derivatives so as to obtain a direction of update $\eps$ that has the largest cosine with the gradient.

\begin{claim}[Optimal direction $\epsilon$]\label{claim:optimal}
The direction $\eps$ which has the best cosine with $\tri f(x)$ in the hyper plane spanned by $\eps_i$ is the projection of $\tri f(x)$ in it. That is, $\eps = \sum_i\ls\tri f(x), \hat{\eps_i}\rs\hat{\eps_i}$. In particular, the cosine squared is given by $\ls\hat{\tri} f(x), \hat{\eps}\rs^2 = \sum_i\ls\hat{\tri} f(x), \hat{\eps_i}\rs^2$.
\end{claim}

\begin{proof}
This is a simple application of the Cauchy-Schwarz inequality. We can write $\eps = \sum_i \alpha_i\hat{\eps_i}$. Denote by $\tri f_{\|}(x)= \sum_i\ls\tri f(x), \hat{\eps_i}\rs\hat{\eps_i}$ the projection of $\tri f(x)$ in the hyper plane spanned by $\eps_i$.
Then, we have: 
\begin{equation}
\ls\tri f(x), \eps\rs = \ls\tri f_{\|}(x), \eps\rs\leq \|\tri f_{\|}(x)\|\|\eps\|
\end{equation}
by Cauchy-Schwarz where we have equality only if $\eps$ and $\tri f_{\|}(x)$ have the same direction. In particular, in this case the cosine is 
\begin{equation}
\ls\hat{\tri} f(x), \hat{\eps}\rs^2 = \frac{\|\tri f_{\|}(x)\|^2}{\|\tri f(x)\|^2} = \sum_i\ls\hat{\tri} f(x), \hat{\eps_i}\rs^2
\end{equation}

\end{proof}

The above statement applies in general given directions $\eps_i$. Usually, we select the $\eps_i$ as random directions. However, if we have access to a direction that we know correlates more strongly to the gradient than a random one,  we can then replace one $\eps_i$ by this direction. In particular, we can simply use the previous update direction in place of one of the random directions $\eps_i$. If it correlates more with the gradient than a random direction, the (expected) value of the cosine squared will be larger. Moreover, note that the claim also implies that we can replace all directions $\eps_i$ by a single $\eps$. For simplicity of presentation, we replace all random directions used in time step $t$ by a single direction $\eps_t$. In this way, we can state the (greedy) optimal update we can do, including the previous update direction. Denote by $\zeta_t$ the update at time $t$, that is $x_{t+1} = x_t + \zeta_t$. We assume, motivated by Claim~\ref{claim:optimal}, that $\zeta_t$ is given by a linear combination of the previous update $\zeta_{t-1}$ and new random samples (orthogonal to $\zeta_{t-1}$) collapsed into a direction $\eps_t$. That is,

\begin{equation}\label{eq:update}
    \zeta_t = \langle \bigtriangledown f_t, \hat{\zeta}_{t-1}\rangle \hat{\zeta}_{t-1} + \langle \bigtriangledown f_t, \hat{\epsilon}_t \rangle \hat{\epsilon}_t . \ 
\end{equation}

As a consequence of Claim~\ref{claim:optimal}, the cosine squared evolves over time as
\begin{equation} \label{eq:cos}
\ls \htri f_t, \hat{\zeta}_{t}\rs ^2=\ls \htri f_t, \hat{\zeta}_{t-1}\rs ^2 + \ls \htri f_t, \hat{\eps}_{t}\rs ^2.
\end{equation}

To showcase the strength of the above update step, let's consider the case where $f$ is a linear function. In this case, because the gradient does not change, the cosine squared is monotonically increasing over time. In particular, if
$X_t = \ls \htri f ,\hzeta_t\rs$ we can write $X_t^2 = X_{t-1}^2 + \ls \htri f, \hat{\eps}_{t}\rs ^2$. We can split $\htri f= \tri f _{\perp\zeta} +\tri f _ { \|\zeta}$ into an orthogonal to $\hzeta_{t-1}$part and a parallel to $\hzeta_{t-1}$ part. Observe that $\ls \htri f, \hat{\eps}_{t}\rs ^2 = \ls \tri f_ {\perp\zeta}, \heps_t\rs^2 = (1-X_{t-1}^2)\ls \htri f_{\perp\zeta}, \hat{\eps}_{t}\rs ^2$, due to the fact that $\|\tri f_{\perp\zeta}\|^2 = 1-X_{t-1}^2$. This implies that $X_t^2 = X_{t-1}^2 + (1-X_{t-1}^2)\ls \htri f_{\perp\zeta}, \hat{\eps}_{t}\rs ^2$, which implies that the cosine increases every time step in expectation by a factor that depends on the cosine squared between a random vector and a fixed unit vector.


\begin{theorem}[Convergence rate for linear functions]\label{thm:convergence-rate-linear}
Let $c$ be a constant such that the expected cosine squared between a random vector and unit one in an $N-1$-dimensional space is $\frac{c}{N-1}$. Let $X_t= \ls \htri f ,\hzeta_t\rs $ be the random variable that denotes the cosine between $\zeta_t$ and $\tri f_t$ at time $t$.
Then, the expected drift of $X_t^2$ is $\mathbb{E}[X_t^2- X_{t-1}^2|X_{t-1}=x_{t-1}]=  (1-x_{t-1}^2)\frac{c}{N-1} $. Moreover, let $\eps>0$ and  define  $T$ to be the first point in time $t$ with $X_t^2\geq 1 - \delta$.  It holds
\begin{equation}
    \mathbb{E}[T]\leq \frac{N-1}{c} \min \{ \frac{1-\delta}{\delta},1+ \ln(1/ \delta)\} \ .
\end{equation}{}
\end{theorem}{}

The first bound $\mathbb{E}[T]\leq \frac{N-1}{c}\frac{1-\delta}{\delta}$ is tight for $\delta$ close to $1$ and follows by an additive drift theorem, while the second bound $\mathbb{E}[T]\leq \frac{N-1}{c}(1+\ln (1/\delta))$ is tight for $\delta $ close to $0$ and follows by a variable drift theorem.
Both drift theorems are taken from \cite{lengler2018drift} and are restated in Section~\ref{sec:drift-theorems}.

Observe that one needs $N$ orthogonal directions to perfectly estimate the gradient. The above result gives a bound with an extra $\ln(1/ \delta)$ factor multiplying $N$. This is because we lose some information when we replace the past sampled update directions by a single one, as new random samples are taken from a larger dimensional space.

Naturally, the linear case is not the most interesting one. We will now analyze the general case, where the gradient is changing every time step. Intuitively, the idea is simple. We have $\ls \htri f_t, \hat{\zeta}_{t}\rs ^2=\ls \htri f_t, \hat{\zeta}_{t-1}\rs ^2 + \ls \htri f_t, \hat{\eps}_{t}\rs ^2$, and as before we can write $\ls \htri f_t, \hat{\eps}_{t}\rs ^2 = (1-\ls \htri f_t, \hat{\zeta}_{t-1}\rs ^2)\ls \htri f_{\perp\hzeta_{t-1}}, \hat{\eps}_{t}\rs ^2$ and note that over the cosine between the previous update direction and the current gradient we add a factor that depends on the expectation between a random vector and a unit one in an $N-1$ dimensional space. To understand how the cosine evolves we need to analyze how $\ls \htri f_t, \hat{\zeta}_{t-1}\rs ^2$ corresponds to $\ls \htri f_{t-1}, \hat{\zeta}_{t-1}\rs ^2$.

To that end, we set $\alpha_t = \ls \htri f_t, \htri f_{t-1}\rs$ and write $\htri f_t = \alpha_t\htri f_{t-1} + \tri f_{\perp}$ where $\tri f_{\perp}$ is orthogonal to $\htri f_t$ and has norm $1-\alpha_t^2$.
Then, the first term of \eqref{eq:cos} is equal to
\begin{align}
    \ls \htri f_t, \hzeta _{t-1}\rs ^2 
    = \ls \alpha_t\htri f_{t-1} + \tri f_{\perp}, \hzeta_{t-1}\rs^2
    = \left(\alpha_t \ls\htri f_{t-1}, \hzeta_{t-1}\rs + \ls\tri f_{\perp}, \hzeta_{t-1}\rs\right)^2 \ .
\end{align}

Therefore, the value of $x_t$ depends on $x_{t-1}$, $\alpha_t$, and $\ls\tri f_{\perp}, \hzeta_{t-1}\rs$.
Write $\hzeta_{t-1}= \zeta_{\|}+\zeta_{\perp}$, where $\zeta_{\|}= x_{t-1} \htri f_{t-1}$ is the parallel part to $\htri f_{t-1}$  and $\zeta_{\perp}= \hzeta_{t-1} - \zeta_{\|}$ is the orthogonal part to $ \htri f_{t-1}$ with squared norm $1-x_{t-1}^2$. The term $\ls \tri f_{\perp}, \hzeta_{t-1}\rs$ can be correlated between time steps which makes an analysis hard. Therefore, we assume that $\zeta_{\perp}$ is a random vector with norm $\sqrt{1-x_{t-1}^2}$ from the subspace orthogonal to $\tri f_{t-1}$.

\begin{theorem}
Let $1\geq x_{t-1}\geq0$, $\zeta_{\perp}$ be a random vector of norm $\sqrt{1-x_{t-1}^2}$ in the subspace orthogonal to $\tri f_{t-1}$ and $\hzeta_{t-1}= x_{t-1}\htri f_{t-1} + \zeta_{\perp}$. Choose $\zeta_t$ according to Equation~\eqref{eq:update}. Then,
\begin{equation*}
    \mathbb{E}[x_t^2|x_{t-1}] = \left(\alpha_t^2x_{t-1}^2 + (1-\alpha_t^2)(1-x_{t-1}^2)\frac{c}{N-1}\right)\left(1-\frac{c}{N-1}\right) + \frac{c}{N-1}\ .
\end{equation*}
\end{theorem}

The evolution of the cosine in the general case depends heavily on the cosine $c_1$ between consecutive gradients. In general, though, this is not a good upper bound and the evolution of the cosine is heavily task dependent. We perform an experiment on MNIST simulating the above theory and our algorithm to analyze how the correlation of the terms $\ls \Delta_{\perp}, \hzeta_{t-1}\rs$ evolves across time steps.










\subsection{Evolution of cosine for general functions depending on the Hessian}
Define $X_t= \ls \htri f_t, \hzeta_t \rs$ to be the cosine between true gradient and update step at time $t$. Here, we are interested how $X_t$ evolves over time $t$. Especially, we are interested in the magnitude of $\mathbb{E}[X_t|X_{t-1}=x_{t-1}]$. 
Recall that by Theorem~\ref{thm:optimal-alpha} it holds
\begin{equation} \label{eq:x_t}
    x_t^2= \ls \htri f_t, \hzeta_{t-1}\rs^2 + \ls \htri f_t, \heps_t\rs^2 \ . 
\end{equation}

We define $\Delta_t$ to be the change of the gradient from time $t-1$ to $t$:
\begin{equation}
    \Delta_t \coloneqq \htri f_t- \htri f_{t-1}
\end{equation}{}
We partition $\Delta_t= c_1 \tri f_{t-1}+ \Delta_{\perp}$, where $\Delta_{\perp}= \Delta_t - \ls \Delta_t, \htri f_{t-1}\rs \htri f_{t-1}$ 
is the part of $\Delta_t$ that is orthogonal to $\tri f_{t-1}$. 
Then, the first term of \eqref{eq:x_t} is equal to
\begin{align}
    \ls \htri f_t, \hzeta _{t-1}\rs ^2 
    = \frac{\ls(1+c_1)\tri f_{t-1} + \Delta_{\perp}, \hzeta_{t-1}\rs^2}{\|\tri f_t \|^2_2}
    =\frac{\left((1+c_1)\|\tri f_{t-1}\| \ls\htri f_{t-1}, \hzeta_{t-1}\rs + \ls \Delta_{\perp}, \hzeta_{t-1}\rs\right)^2}{(1+c_1)\|\tri f_{t-1}\|^2 + \|\Delta_{\perp}\|^2} \ , 
\end{align}
and since $\heps_t$ is orthogonal to $\zeta_{t-1}$, the second term of \eqref{eq:x_t} is equal to
\begin{align}
\ls \htri f_t, \heps _{t}\rs ^2 &= \ls \tri f _ { \perp\hzeta_{t-1}}, \heps_t \rs^2 = 
    \left(1-\ls \htri f_t, \hzeta_{t-1} \rs^2\right) \ls \htri f _ { \perp\hzeta_{t-1}}, \heps_t \rs^2 \ .
\end{align}{}
Therefore, the value of $x_t$ depends on $x_{t-1}$, $c_1$, $\|\Delta_{\perp}\|$, $\|\tri f_t\|$ and $\ls \Delta_{\perp}, \hzeta_{t-1}\rs$. 
Write $\hzeta_{t-1}= \zeta_{\|}+\zeta_{\perp}$, where $\zeta_{\|}= x_{t-1} \htri f_{t-1}$ is the parallel to $\htri f_{t-1}$ part and $\zeta_{\perp}= \hzeta_{t-1} - \zeta_{\|}$ is the orthogonal to $ \htri f_{t-1}$ part. 
The term $\ls \Delta_{\perp}, \hzeta_{t-1}\rs$ can be correlated between time step which makes an analysis hard or maybe impossible. Therefore, we assume that 
$\zeta_{\perp}$ is a random vector with norm $\sqrt{1-x_{t-1}^2}$ from the subspace orthogonal to $\tri f_{t-1}$. 

\begin{theorem}
Let $1\geq x_{t-1}\geq0$, $\zeta_{\perp}$ be a random vector of norm $\sqrt{1-x_{t-1}^2}$ in the subspace orthogonal to $\tri f_{t-1}$ and $\hzeta_{t-1}= x_t\htri f_{t-1} + \zeta_{\perp}$. Choose $\zeta_t$ according to Equation~\eqref{}. 
Then, 
\begin{equation*}
    \mathbb{E}[x_t^2]= 
\end{equation*}{}
\end{theorem}{}






\subsection{Old version of Section 6.3}

We write the new gradient as $\tri f_t = \tri f_{t-1} +\Delta_t $. Note that the first order approximation of $\Delta_t$ is given by 
\begin{equation}\label{\eq:Delta}
    \Delta_t\approx H \zeta_{t-1}= H  (\ls \tri f_{t-1}, \hzeta_{t-2}\rs \hzeta_{t-2} + \ls \tri f_{t-1}, \heps_{t-1} \rs \heps_{t-1} ) \ , 
\end{equation}{}
where $H$ is the Hessian of $f$ at point $x_{t-1}$. 
For the following calculations we require that $\Delta_t$ relates to the plane spanned by $\tri f_{t-1}$ and $\zeta_{t-1}$ like a random vector. Therefore, we assume that $\Delta_t \sim \mathcal{N}(0,\Sigma)$, where  the covariance matrix $\Sigma$ is the $N$-dimensional diagonal matrix with diagonal entries equal to $\sigma^2= \frac{\|\Delta_t\|^2}{N}$. This assumption implies that $\Delta_t$ has in expectation the correct norm. 
We remark that this assumption is of course not true in general. However, as the Hessian $H$ is  unspecified and the $\zeta_{t-1}$ is a noisy estimate of $\tri f_t$, the assumption seems reasonable and enables a mathematical analysis of the process.
We write $\Delta_t= c_1 \tri f_{t-1}+ \Delta_{\perp} $ as an parallel to $\tri f_{t-1}$ part and and orthogonal to $\tri f_{t-1}$ part. Note that $c_1$ is a $\mathcal{N}(0,\frac{\sigma^2}{\|\tri f_{t-1}\|^2})$ distributed random variable. 
Moreover, $\mathbb{E}[\|\Delta_{\perp}\|^2_2]=\mathbb{E}[\|\Delta_t\|^2_2- \|c_1\tri f_{t-1}\|_2^2]=N\sigma^2-\sigma^2=(N-1)\sigma^2$. We assume that $\|\Delta_{\perp}\|^2_2=(N-1)\sigma^2$. 
This approximation is reasonable as $\|\Delta_{\perp}\|^2_2$ is the sum of $N-1$ independent Gaussian variables and thus heavily concentrated. 
Then it holds that $\|\tri f_t\|^2_2= (1+c_1)^2 \|\tri f_{t-1}\|^2_2+ (N-1)\sigma^2$.
By Theorem~\ref{thm:optimal-alpha}, it holds that $\ls \htri f_t, \hzeta_{t}\rs^2= \ls \htri f_t, \hzeta_{t-1}\rs^2 + \ls \htri f_t, \heps_t\rs ^2$. We are going to compute both parts of the right hand side. In order  to compute the expectation of $ \ls \htri f_t, \hzeta _{t-1}\rs ^2 $ over the random choice of $\Delta_{\perp}$, we split $\hzeta_{t-1}= \zeta_{\|}+\zeta_{\perp}$, where $\zeta_{\|}= \ls \htri f_{t-1}, \hzeta_{t-1}\rs \htri f_{t-1}$ is the parallel to $\htri f_{t-1}$ part and $\zeta_{\perp}= \hzeta_{t-1} - \zeta_{\|}$ is the orthogonal to $ \htri f_{t-1}$ part. Further, we define $x_t= \ls \htri f_t, \hzeta_t\rs$ to be the cosine at time $t$, which implies $\|\zeta_{\|}\|^2= x_{t-1}^2$ and $\|\zeta_{\perp}\|^2= 1-x_{t-1}^2$. 

\begin{align}
    & \mathbb{E}_{\Delta_{\perp}}[\ls \htri f_t, \hzeta _{t-1}\rs ^2 ]\\
    &= \mathbb{E}_{\Delta_{\perp}}\left[ \frac{\ls(1+c_1)\tri f_{t-1} + \Delta_{\perp}, \hzeta_{t-1}\rs^2}{\|\tri f_t \|^2_2}\right]\\
    &=\mathbb{E}_{\Delta_{\perp}}\left[ \frac{(1+c_1)^2\|\tri f_{t-1}\|^2 \ls \htri f_{t-1}, \hzeta_{t-1}\rs^2 + 2  (1+c_1)\|\tri f_{t-1}\|\ls \htri f_{t-1}, \hzeta_{t-1}\rs \ls \Delta_{\perp},\zeta _{\perp}\rs + \ls \Delta_{\perp}, \zeta_{\perp}\rs^2}{\|\tri f_t\|^2_2} \right]\\
    &= \frac{(1+c_1)^2 \|\tri f_{t-1}\|^2x_{t-1}^2+ \sigma^2\|\zeta_{\perp}\|^2}{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}\\
    &= \frac{(1+c_1)^2 \|\tri f_{t-1}\|^2x_{t-1}^2+ (1-x_{t-1}^2)\sigma^2 }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}\ , 
\end{align}
where we used that  $\ls\Delta_{\perp}, \zeta_{\perp}\rs$ is independent of $c_1$, that $\mathbb{E}[\ls\Delta_{\perp}, \zeta_{\perp}\rs]=0$ and that $\mathbb{E}[\ls\Delta_{\perp}, \zeta_{\perp}\rs^2]=\|\zeta_{\perp}\|^2\sigma^2$. 

Next, we compute the expectation of $\ls \htri f_t, \heps_t \rs^2$. Because $\heps_t$ is chosen orthogonal to $\hzeta_{t-1}$, we split $\htri f_t$ into a part orthogonal to $\hzeta_{t-1}$ and a part parallel to $\hzeta_{t-1}$. By that, we get $\htri f_t = \ls \htri f_t, \hzeta_{t-1} \rs \htri f _{\|\hzeta_{t-1}} +\tri f _ { \perp\hzeta_{t-1}}$, where $\|\tri f _ { \perp\hzeta_{t-1}}\|^2 = 1-\ls \htri f_t, \hzeta_{t-1} \rs^2$. Now we can compute the expectation:

\begin{align}
    \mathbb{E}_{\Delta_{\perp}, \heps_{t}}[\ls \htri f_t, \heps _{t}\rs ^2 ]&= \mathbb{E}_{\Delta_{\perp},\heps_{t}}\left[ \ls \tri f _ { \perp\hzeta_{t-1}}, \heps_t \rs^2\right]\\
    &= \mathbb{E}_{\Delta_{\perp},\heps_{t}}\left[\left(1-\ls \htri f_t, \hzeta_{t-1} \rs^2\right) \ls \htri f _ { \perp\hzeta_{t-1}}, \heps_t \rs^2\right]\\
    &= \mathbb{E}_{\Delta_{\perp}}\left[\left(1-\ls \htri f_t, \hzeta_{t-1} \rs^2\right) \mathbb{E}_{\heps_{t}}\left[ \ls \htri f _ { \perp\hzeta_{t-1}}, \heps_t \rs^2\right]\right]\\
    &= \mathbb{E}_{\Delta_{\perp}}\left[\left(1-\ls \htri f_t, \hzeta_{t-1} \rs^2\right) \frac{c}{N-1}\right]\\
    &= \left(1 - \frac{(1+c_1)^2 \|\tri f_{t-1}\|^2x_{t-1}^2+ (1-x_{t-1}^2)\sigma^2 }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}\right)\frac{c}{N-1}\\
    &= \left(1 - x_{t-1}^2 - \frac{-(N-1)\sigma^2x_{t-1}^2+ (1-x_{t-1}^2)\sigma^2 }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}\right)\frac{c}{N-1}    
\end{align}

where we used that $\mathbb{E}_{\Delta_{\perp}}[\ls \htri f_t, \hzeta _{t-1}\rs ^2 ]= \frac{(1+c_1)^2 \|\tri f_{t-1}\|^2x_{t-1}^2+ (1-x_{t-1}^2)\sigma^2 }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}$ and that the expected cosine squared between a unit vector and a random one is $\frac{c}{N-1}$. 

\iffalse
Further, denote by $\tri f_{\perp\zeta}$  the part of $\tri f_{t-1}$ that is orthogonal to $\hzeta_{t-1}$. Note that $\ls \tri f_{t-1}, \heps_t\rs= \ls \tri f_{\perp\zeta}, \heps_t\rs= \|\tri f_{t-1} \|^2(1-x_{t-1}^2) \ls \htri f_{\perp\zeta}, \heps_t\rs $.

Now we are ready to compute the expectation of $\ls \htri f_t, \heps_{t}\rs$ over the random choice of $\Delta_{\perp}$ and $\heps_{t}$.
\begin{align}
    \mathbb{E}_{\Delta_{\perp}, \heps_{t-1}}[\ls \htri f_t, \heps _{t-1}\rs ^2 ]&= \mathbb{E}_{\Delta_{\perp},\heps_{t-1}}\left[ \frac{\ls(1+c_1)\tri f_{t-1} + \Delta_{\perp}, \heps_{t-1}\rs^2}{\|\tri f_t \|^2_2}\right]\\
    &=\mathbb{E}_{\Delta_{\perp},\heps_{t-1}}\left[ \frac{(1+c_1)^2\ls \tri f_{t-1}, \heps_{t-1} \rs^2 + 2  (1+c_1)\ls \tri f_{t-1}, \heps_{t-1} \rs \ls \Delta_{\perp}, \heps _{t-1}\rs + \ls \Delta_{\perp}, \heps_{t-1}\rs^2}{\|\tri f_t\|^2_2} \right]\\
    %&= \frac{(1+c_1)^2 \| \tri f_{t-1}\|^2 (1-x_{t-1}^2)\frac{1}{N-1}+  \|\Delta_{\perp}\|^2\left(1-(1-x_{t-1}^2)\frac{1}{N-1}\right) \frac{1}{N-1} }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2} \\
    & \approx \frac{(1+c_1)^2 \| \tri f_{t-1}\|^2 (1-x_{t-1}^2)\frac{1}{N-1}+  \|\Delta_{\perp}\|^2 \frac{1}{N-1} }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2} \ .
\end{align}{}
\fi

We can now compute the expected value of $\ls \htri f_t, \hzeta _{t-1}\rs ^2$ over $\Delta$ by taking the expectation first over $\Delta_{\perp}$ and then over $c_1$.
\begin{align}
    \mathbb{E}_{\Delta}[\ls \htri f_t, \hzeta _{t-1}\rs ^2 ] &= \mathbb{E}_{c_1}\left[\mathbb{E}_{\Delta_{\perp}}[\ls \htri f_t, \hzeta _{t-1}\rs ^2 ]\right]\\
    &= \mathbb{E}_{c_1}\left[\frac{(1+c_1)^2 \|\tri f_{t-1}\|^2x_{t-1}^2+ (1-x_{t-1}^2)\sigma^2 }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}\right]\\
    &= x^2_{t-1} + \mathbb{E}_{c_1}\left[\frac{-(N-1)\sigma^2x^2_{t-1}+ (1-x_{t-1}^2)\sigma^2 }{(1+c_1)^2\|\tri f_{t-1}\|^2+ (N-1)\sigma^2}\right].
\end{align}

By combining the above expressions, we can compute the expected value of the cosine squared:
\begin{align*}
    & \mathbb{E}[x_t^2]\\
    &=\mathbb{E}[\ls \htri f_t, \hzeta_{t-1}\rs^2 + \ls \htri f_t \heps_t\rs^2]\\
    &=x_{t-1}^2 + (1-x_{t-1}^2)\frac{c}{N-1} + \left(1-\frac{c}{N-1}\right)\mathbb{E}_{c_1}\left[ \frac{-(N-1)\sigma^2 x_{t-1}^2 + \sigma^2(1-x_{t-1}^2) }{(1+c_1)^2\|\tri f_{t-1}\|^2 + (N-1)\sigma^2}\right]\\
    &\approx    x_{t-1}^2 + (1-x_{t-1}^2)\frac{c}{N-1}  + \left(1-\frac{c}{N-1}\right)\frac{-(N-1)\sigma^2 x_{t-1}^2 + \sigma^2(1-x_{t-1}^2) }{\|\tri f_{t-1}\|^2 + (N-1)\sigma^2}\\
    &= x_{t-1}^2 + 
    \frac{\frac{c\|\tri f_{t-1}\|^2}{N-1}+(1+c-\frac{c}{N-1})\sigma^2 - \left(\frac{c\|\tri f_{t-1}\|^2}{N-1} +(N-\frac{c}{N-1})\sigma^2\right)x_{t-1}^2}
    {\|\tri f_{t-1}\|^2 + (N-1)\sigma^2} \ .
\end{align*}{}

Note that for any given value $x_{t-1}^2$ the last term gives us the drift. The drift is positive if 
\begin{equation}
     A \coloneqq \frac{\frac{c\|\tri f_{t-1}\|^2}{N-1}+(1+c-\frac{c}{N-1})\sigma^2}{\frac{c\|\tri f_{t-1}\|^2}{N-1} +(N-\frac{c}{N-1})\sigma^2} \geq x_t^2
\end{equation}
and negative otherwise. Therefore, $x_t$ converges to $A$, which we are going to estimate in the following.

 Define $\bar{\zeta}_{t-1}= \ls \htri f_{t-1}, \hzeta_{t-2}\rs \hzeta_{t-2} + \ls \htri f_{t-1}, \heps_{t-1} \rs \heps_{t-1}$.
By Equation \eqref{eq:Delta}, it holds 
\begin{equation}
    \|\Delta_t\|\approx \|H\zeta_{t-1} \| =
    \|\tri f_{t-1}\| \cdot \| H \bar{\zeta}_{t-1}\| \leq \|\tri f_{t-1}\| \cdot \| H\|_{op}  \ , 
\end{equation}{}
where $\|H\|_{op}$ is the operator norm of $H$ and $\|\bar{\zeta}_{t-1}\|\leq 1$ follows by the orthogonality of $\hzeta_{t-2}$ and $\heps_{t-1}$. Recall that $\sigma^2= \frac{\|\Delta_t\|^2}{N}= \frac{\|\tri f_{t-1}\|^2\cdot \|H\bar{\zeta}_{t-1}\|^2}{N}$. 
Plugging this in, we obtain

\begin{align}
    A&= \frac{c + (1+c-\frac{c}{N-1})\frac{N-1}{N}\|H\bar{\zeta}_{t-1}\|^2}{c+ (N-\frac{c}{N-1})\frac{N-1}{N}\|H\bar{\zeta}_{t-1}\|^2} \\
    &= \frac{1+c- \frac{c}{N-1}}{N-\frac{c}{N-1}}+ \frac{c(1-\frac{1+c-\frac{c}{N-1}}
    {N-\frac{c}{N-1}})}
    {c + (N-\frac{c}{N-1})\frac{N-1}{N}\|H\bar{\zeta}_{t-1}\|^2}\\
     &= \frac{1+c- \frac{c}{N-1}}{N-\frac{c}{N-1}}+ \frac{c(1-\frac{1+c-\frac{c}{N-1}}
    {N-\frac{c}{N-1}})}
    {c + (N-\frac{c}{N-1})\frac{N-1}{N}\|H\|_{op}^2}
\end{align}{}

Note that $A$ tends to $1$ as $\|H\|_{op}$ to $0$, which is in line with Theorem~\ref{thm:convergence-rate-linear}. Moreover, $A$ tends to $\frac{1+c-\frac{c}{N-1}}{N-\frac{c}{N-1}}$ in the limit of $\|H\|_{op}$ tending to $\infty$.

